Topological Properties and Temporal Dynamics of Place Networks in Urban Environments

Understanding the spatial networks formed by the trajectories of mobile users can be beneficial to applications ranging from epidemiology to local search. Despite the potential for impact in a number of fields, several aspects of human mobility networks remain largely unexplored due to the lack of large-scale data at a fine spatiotemporal resolution. Using a longitudinal dataset from the location-based service Foursquare, we perform an empirical analysis of the topological properties of place networks and note their resemblance to online social networks in terms of heavy-tailed degree distributions, triadic closure mechanisms and the small world property. Unlike social networks however, place networks present a mixture of connectivity trends in terms of assortativity that are surprisingly similar to those of the web graph. We take advantage of additional semantic information to interpret how nodes that take on functional roles such as `travel hub', or `food spot' behave in these networks. Finally, motivated by the large volume of new links appearing in place networks over time, we formulate the classic link prediction problem in this new domain. We propose a novel variant of gravity models that brings together three essential elements of inter-place connectivity in urban environments: network-level interactions, human mobility dynamics, and geographic distance. We evaluate this model and find it outperforms a number of baseline predictors and supervised learning algorithms on a task of predicting new links in a sample of one hundred popular cities.

==> conclusion.tex <==
In this work, we have investigated the properties of urban place networks formed by the check-in patterns of millions of Foursquare users across a large set of $100$ cities around the globe.
We have shown that these networks exhibit many of the well-known properties of other social and technological networks, and that the growth patterns of these networks are characterized by a dynamic edge generation process over a relatively stable set of nodes.  In the light of the volatility of these networks, we presented a number of models that exploit both network structure and mobility information about Foursquare users in order to better predict the links that will appear in the network during future periods. We discussed the performance of those models, and found that 
a novel gravity model which combines network, mobility and geographic signals performs best on the link prediction task, with minimal parametrization requirements 
and computation costs.

% In terms of future work, we are planning to explore the link prediction task in a real-time setting, developing models that are able to respond to anomalous activity in the network that can arise for example when large social events form in cities.  Along these lines, it would be interesting to predict how certain events in a city disrupt the mobility networks, such as closing a major transportation hub or opening a new sports arena. Another interesting direction for future work is to explore the networks emerging on larger geographic scales than that of a single city, instead looking at the connectivity and flow of users between cities and countries as well.  Finally, we are motivated to better connect work on link prediction in urban place networks with predicting individual patterns of mobility.

